Learning Bayesian Networks in the Presence of Structural Side Information

We study the problem of learning a Bayesian network (BN) of a set of variables when structural side information about the system is available. It is well known that learning the structure of a general BN is both computationally and statistically challenging. However, often in many applications, side information about the underlying structure can potentially reduce the learning complexity. In this paper, we develop a recursive constraint-based algorithm that efficiently incorporates such knowledge (i.e., side information) into the learning process. In particular, we study two types of structural side information about the underlying BN: (I) an upper bound on its clique number is known, or (II) it is diamond-free. We provide theoretical guarantees for the learning algorithms, including the worst-case number of tests required in each scenario. As a consequence of our work, we show that bounded treewidth BNs can be learned with polynomial complexity. Furthermore, we evaluate the performance and the scalability of our algorithms in both synthetic and real-world structures and show that they outperform the state-of-the-art structure learning algorithms.

==> coverletter.tex <==
\clearpage
\section*{NeurIPS-21 Submission}

\paragraph{The paper ID of the NeurIPS-21 submission:} 
Paper 6876


\paragraph{The authors listed on the NeurIPS-21 submission:}
\begin{itemize}
    \item Ehsan Mokhtarian
     \item Sina Akbari 
     \item Fateme Jamshidi
     \item Jalal Etesami
     \item Negar Kiyavash
\end{itemize}


\paragraph{The title of the NeurIPS-21 submission:}
 Learning Bayesian Networks in the Presence of Structural Side Information

\section*{NeurIPS-21 reviews \& detailed response to each point raised by reviewers}
Herein, we present all the NeurIPS-21 reviews, our detailed response to each point raised by the reviewers, and describe all changes we have made since the NeurIPS-21 submission. 
Please note that all references and citations in NeurIPS-21 reviewers' comments are with respect to our neurips submission (It has different numbering that our AAAI22 submission) which is attached.


\subsection*{Reviewer 1:}
\textbf{Summary:}
In this work, the authors describe a general recursive framework for constraint-based Bayesian network (BN) structure learning. They then provide two instantiations of the framework which take advantage of structural constraints, namely diamond-free and max clique size, to reduce the required number of conditional independence (CI) tests. Worst-case complexity analysis shows that the proposed approach requires fewer CI tests than similar approaches which do not use such constraints. A limited set of empirical results suggests the approach outperforms baseline methods.
\\
\\
\textbf{Main Review:}
--- Originality:
The proposed work is modestly novel. As the authors point out, the general recursive framework for bounding the size of CI tests was previously described in [21] (though there does not appear to be a currently-published, peer-reviewed version of that article out, yet). To the best of my knowledge, prior work has also not considered the exact structural constraints in this work. As described in “Significance” and “Limitations,” though, the motivation for such constraints seems somewhat limited.

--- Quality:
I did not verify the proofs of this work in detail; however, the technical quality of the algorithmic and theoretical work seem high (though see below about Algorithm 4). On the other hand, the empirical evaluation is limited and does shed much insight into when the approach works well and when it does not.

--- Clarity: 
While the language of the paper is generally quite clear, the paper has several limitations concerning the clarity of the technical contributions. First, the main text does not provide any intuition on the proofs of the correctness and complexity of the approach. Additionally (discussed more in “Limitations”), there is a very confusing paragraph about the validity of Algorithm 4; the main text does not really revisit this either theoretically or empirically to clarify the implications.

--- Significance: 
As hinted in “Originality,” I believe the impact and significance of the current work may be limited. The general idea of a recursive CI-based BN learning has been previously proposed several times (e.g., [Yehezkel and Lerner, JMLR 2009], ref. [21] in the paper). As described in “Limitations”, it is not clear that diamond-free structures are common in real data. Additionally, compared to bounded treewidth, the motivation for bounded clique number seems limited.
\\
\\
\textbf{Limitations And Societal Impact:}
--- Significance:
Both of the considered structural constraints seem to have limitations. While the authors show that diamonds may not be likely in certain types of random graph structures, structures for actual data often contain particular motifs [Alon, Nature Review Genetics 2007; Bois and Gayraud, Journal of Computational Biology 2015]. Thus, it is less clear how meaningful such a constraint may be, especially a priori.

The motivation for bounded clique numbers also seems limited. In comparison, learning a bounded treewidth Bayesian network guarantees that inference in that network will have bounded complexity. It is not obvious to me that bounded clique size would offer any kind of similar guarantees.

--- Clarity:
As mentioned above, the main text does not include any intuition or high-level description of the proofs of the main results in the paper. The length and technical detail in the appendices make clear that the results are not obvious. Nevertheless, these are needed to justify the main theoretical contributions of this work. Thus, some brief overview of these should appear in the main text.

My second major concern about the clarity of the work concerns the last paragraph of Section 4, which raises some points about the validity of Algorithm 4 in cases where the underlying structure includes diamonds. It is unclear to me why the algorithm may still output a graph containing diamonds in this case. The appendices do not appear to address this issue from a theoretical perspective, and this is also not explored empirically in any detail. Thus, it is not clear to me how serious of a concern this limitation actually is.

--- Quality:
As mentioned above, the empirical evaluation does not reveal much about the proposed algorithms. For example, the bounded clique version of RSL consistently has a worse F1 score than the diamond version, but the experiments do not suggest any explanation. Further, it is not clear how sensitive the bounded clique version is to the choice of clique size. Additionally, the experiments do not systematically explore the behavior of the algorithms when their assumptions are violated; for example, $RSL_D$ seems to do well on Andes even though it includes diamonds. Finally, the experiments only consider relatively large dataset sizes (50*n); they do not examine the algorithms in limited data scenarios where the independence tests are less reliable.

Confidence intervals should be given on the measurements. The performances of several methods are similar, and it is difficult to tell if any of the results are significant.

--- Minor comments, typos, etc:
The references are not consistently formatted.

The competing algorithms considered in the experimental section are not particularly representative of the state of the art. I appreciate that the contribution of this work is mostly theoretical; however, to convincingly argue for the empirical value of the approach, it would be helpful to include a few modern approaches besides MARVEL (e.g., https://www.bnlearn.com/documentation/man/constraint.html for more constraint-based methods).

Several of the methods appear to be missing in Figure 2. For example, $RSL_D$ does not appear to be in Figure 2(d). Presumably, the runs out of resources, but this should be clarified.

“perquisites” -> “prerequisites” (Appendix B)

--- Societal Impact:
No obvious, direct societal impact.
\\
\\
\textbf{Ethical Concerns:}
No ethical concerns.
\\
\\
\textbf{Needs Ethics Review:} No
\\
\\
\textbf{Time Spent Reviewing:} 3
\\
\\
\textbf{Rating:} 5: Marginally below the acceptance threshold
\\
\\
\textbf{Confidence:} 3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.
\\
\\
\textbf{Code Of Conduct:} While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.

\subsection*{Detailed response to Reviewer 1 \& corresponding changes:}
Regarding the comments in the Significance part:
\begin{itemize}
    \item 
As the reviewer mentioned, we have studied two structural side information: diamond-free and boundedness of the clique number. 
As we argue in Section 7 {\color{blue}(Section 6 in our NeurIPS-21 submission)} about random graphs, sparse structures are diamond-free with high probability. 
Note that even $K_4$ ({\color{blue}complete graph with four vertices}) is a diamond-free graph, i.e., very dense graphs can also be diamond-free. Moreover, such structures appear frequently in many real-world applications. For instance, we observed this in the main database frequently used to study BNs (https://www.bnlearn.com/bnrepository/). We randomly selected 17 structures from this website for our experiments and observed that 15 were diamond-free. 
Even if the graph is not diamond-free, $RSL_D$ does not necessarily make a mistake. {\color{blue} We added section C in Appendix in which we explain this property in detail}. 
It is still highly likely that $RSL_D$ will choose the right node to remove and learn the structure with no errors (as witnessed by the example of Andes in our experiments). 
It is also worth mentioning that diamond-free graphs are a type of planar graphs that are well-studied in graph theory and possess interesting properties, e.g., while the coloring problem in general graphs is NP-hard, for diamond-free graphs is polynomial-time solvable. This work shows that the complexity of structure learning for such graphs is again polynomial in the number of variables.
 {\color{blue}
 We emphasized these facts in our AAAI-22 submission, Section 6.
 }
 
 \item
We show that side information on the clique number of the graph reduces the learning complexity. It is important to emphasize that our proposed algorithm $RSL_\omega$ can verify the correctness of the bound on the clique number. Therefore, even if the clique number is not known, we can run $RSL_\omega$ with an initial guess about the clique number of the underlying BN. If the clique number of the output graph is less than the initial guess, the graph is learned correctly; otherwise, we need to increase our guess (Thus, as a side product, $RSL_\omega$ can identify the clique number of the underlying structure).
{\color{blue} We added Section 5 in our new submission in which we explain the verifiability of $RSL_\omega$ in Proposition 4 and develop Algorithm 5 that does not require any side information.}
 
 \item
We appreciate the insightful comment about the relationship between our assumption on the clique number and the treewidth in (Elidan and Gould 2008, Korhonen and Parviainen 2015). In fact, we should emphasize that our work \textit{generalizes} the assumption on the treewidth. This is because, in general, the clique number is less than treewidth+1. Hence, having a bound on the treewidth of the underlying structure will lead to a bound on the clique number, and consequently (based on the result of Theorem 1), our algorithm will also have bounded complexity. On the other hand, a bound on the clique number does not translate to a bound in the correct direction for the treewidth. Therefore, the algorithm proposed in (Elidan and Gould 2008) cannot learn the graph with any guarantee. We also emphasize that the algorithm in (Elidan and Gould 2008, Korhonen and Parviainen 2015) requires knowledge of the treewidth, but as we mentioned above, $RSL_\omega$ can identify the structure without knowing the clique number but by progressively guessing and learning it.
{\color{blue} In our AAAI-22 submission, we rigorously explained the relationship between bounded treewidth assumption and our bounded clique number side information in the Introduction section and Related work. Moreover, we added more details on how our proposed $RL_\omega$ can learn bounded treewidth BNs and compared its complexity with the state-of-the-art exact and heuristic algorithms in Related work.
}
 
 \end{itemize}


Regarding the comments in the Clarity part:
\begin{itemize}

\item 
Last paragraph of Section 6 ({\color{blue} Section 4 of our NeurIPS21 submission}): We proved the correctness of Algorithm 4 under the assumption that the underlying structure is diamond-free in Theorem 2 ({\color{blue} Theorem 1 in our NeurIPS21 submission}). However, when the assumption is not valid, the output of Algorithm $RSL_D$ is not necessarily incorrect. More precisely, RSL makes a mistake when either Algorithm 3 incorrectly reports a node as removable or Algorithm 4 identifies the wrong neighbors. For example, Algorithm 3 selects a wrong removable in the left graph in Figure 1 (this graph violates the diamond-free assumption) only when A is selected in the first iteration. Note that this happens with probability 0.25, since all the variables have the same Markov boundary size. Another example is the right graph in Figure 1, in which Algorithm 3 works without error (all the variables are truly removable) but Algorithm 4 incorrectly identifies the neighbors only when nodes B or C are selected by Algorithm 3 in the first iteration. This occurs with probability 0.5. 
{\color{blue} 
In the last paragraph of Section 6 of our AAAI-22 submission, we briefly explained the aforementioned notes to avoid any ambiguity. 
Further, we added more details in Section C of Appendix including Proposition 11 which proofs that $RSL_D$ has no false negative. 
}
\end{itemize}

Experiments:
\begin{itemize}
    \item Large dataset size (50n): We also ran the experiments for various dataset sizes (e.g., 20n) and got similar results. {\color{blue} We have added the results for 20n in Figure \ref{fig: data 0.65}}.
Confidence intervals: As mentioned in Section 8, "Each point is reported as the average of 100 runs, and the shaded areas indicate the 80\% confidence intervals." Performance of various methods: As depicted in Figure 2.a, 
$RSL_D$ outperforms all the algorithms in terms of time complexity and accuracy. It seems that for graphs that are not very sparse, although the graph might contain diamonds, 
$RSL_D$ outperforms the others. One justification for this robustness is that when the graph is not diamond-free, the event that 
$RSL_D$ makes a mistake is quite rare. Moreover, in case of a mistake, 
$RSL_D$ outputs only a few extra edges (It does not miss any edges) in the graph. {\color{blue}To support our claim more rigorously, we added Proposition 11 in the Appendix C that shows even if the underlying BN contains diamonds, the output of $RSL_D$ does not miss any edges i.e.,  $RSL_D$ has recall one.}
\end{itemize}




\subsection*{Reviewer 2:}
\textbf{Summary:}
A constraint-based approach to learning BNs with "side information" is presented. By side information is meant a constraint on the DAG structure. Here the constraints considered are (1) being diamond-free and (2) having an upper bound on clique number.

Having such (known) constraints can inform a learning algorithm: specifically a recursive approach is possible where 'removable' variables can be identified. A DAG vertex with no descendants would be removable, for example, since its removal does not affect the CI relations between the remaining variables. The basic recursive approach builds on earlier work.
\\
\\
\textbf{Main Review:}
The paper is fairly well written. We get theoretical results on complexity. I am not sure how often in real applications, we would actually have this particular sort of side information, but it is good to see reasonably plausible prior knowledge being used. The empirical results fit with the theory and the authors' algorithm compares well empirically as compared to some reasonable alternatives.

Critique:
The various algorithms are presented with an unstated assumption that we are doing oracle-based learning. For example, as noted in the "Problem description" section we do not learn from $P_V$, but from a finite sample drawn from $P_V$. So it is a mistake to state that Algorithm 1 (RSL, the main algorithm) takes $P_V$ as an input. This error is repeated on line 135. Also on line 168: the algorithms mentioned do not "recover the Markov boundaries of a set of random variables". They estimate these Markov boundaries from a finite sample of data. I think some small alteration to the presentation could fix this.

Errors, possibly cumulative ones, from incorrect results of CI test on finite data, are not analysed. There is no empirical comparison of the effect of different significance levels: they always use 0.01 (and $2/n^2$ for Markov blanket "discovery" - actually estimation).

The paper mentions score-based methods, but if I am not mistaken, the comparisons are only with algorithms where Markov boundary estimation is a key component.

Nonetheless the algorithms compared against (in Table 2) are reasonable ones and the authors' method allows a great reduction in CI testing - and the F1 scores are better (sometimes not by a great margin). Also, interestingly, we have good empirical results when the true graph is not diamond-free.

"Runtime and the number of CI tests are reported after Markov boundary discovery". It would be good to know how long Markov boundary estimation takes.

The authors state that side information has been incorporated in score-based methods "in a limited fashion". But score-based methods based on Constraint Programming or Integer Linear Programming allow one to add all sorts of constraints to the DAG learning problem. It would be interesting to compare this approach with a score-based approach which ruled out diamonds and/or bounded clique number. In any score-based approach which had binary variables for both parent sets and adjacencies in the DAG, one would rule out diamonds with simple linear constraints as follows: I(D<-{A,B,C}) + I(A-B) + I(A-C) <= 2 + I(B-C) If cliques of size 4 (and above) were not allowed, one could have constraints such as: I(D<-{A,B,C}) + I(A-B) + I(A-C) + I(B-C) <= 3 I don't know whether this would work well on reasonably-sized problems, since there would have to be very many such constraints (although they could perhaps be added lazily). Also I don't know whether it would make learning easier or harder, but it would be interesting to see.
Fix capitalisation in the refs.
\\
\\
\textbf{Limitations And Societal Impact:}
Societal impact was not addressed.
\\
\\
\textbf{Ethical Concerns:}
No ethical issues.
\\
\\
\textbf{Needs Ethics Review:} No
\\
\\
\textbf{Time Spent Reviewing:} 2
\\
\\
\textbf{Rating:} 7: Good paper, accept
\\
\\
\textbf{Confidence:} 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
\\
\\
\textbf{Code Of Conduct:} While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.


\subsection*{Detailed response to Reviewer 2 \& corresponding changes:}

\begin{itemize}
    \item 
\textit{The various algorithms are presented with an unstated assumption that we are doing oracle-based learning. For example, as noted in the "Problem description" section we do not learn from $P_V$
, but from a finite sample drawn from $P_V$
. So it is a ... I think some small alteration to the presentation could fix this.}

As the reviewer correctly mentioned, structural learning is from data, not the probability distribution in practice. However, in the theoretical part, we present our algorithms and results under the assumption that we have access to an infinite number of sample points or the true joint distribution equivalently. We  emphasized this in the main text to avoid any ambiguity. {\color{blue} We have mentioned that in practice, the finite sample data at hand is used instead of $P_{\OV}$ in Section \ref{sec: RSL}, footnote 6.}


\item 
\textit{There is no empirical comparison of the effect of different significance levels: they always use 0.01 (and $2/n^2$ for Markov blanket "discovery" - actually estimation).}

We ran the algorithms for a wide range of significance levels, and the numbers around 0.01-0.05 work best for almost all the Algorithms. 
\textcolor{red}{We have included the Figure \ref{fig: effect of sig level} in Appendix F to support the fact that the choice of significance level does not alter the experimental results significantly.} 
We also note that this choice of significance level is common in constraint-based methods. Also, as discussed in reference (Pellet and Elis- seeff 2008) of the paper, $2/n^2$ is a good choice for Markov boundary discovery.

\item 
\textit{``Runtime and the number of CI tests are reported after Markov boundary discovery''. It would be good to know how long Markov boundary estimation takes.}


Since all the methods require Markov boundary, and we used a similar method for all of them, the runtime is the same. However, In the method that we used in our experiments, the number of CI tests is always $\binom{n}{2}$, and \textcolor{blue}{as suggested by the reviewer, we reported some of the runtimes in Figure 6 in Appendix F}

\item
\textit{In any score-based approach which had binary variables for both parent sets and adjacencies in the DAG, one would rule out diamonds with simple linear constraints as follows: I(D<-{A,B,C}) + I(A-B) + I(A-C) <= 2 + I(B-C) If cliques of size 4 (and above) were not allowed, ... it would be interesting to see.}


We appreciate the insightful comment of the reviewer. Some score-based algorithms are capable of incorporating structural side information.
{\color{blue} We have reviewed some such related work in our AAAI-22 submission and compared their assumptions and complexity with ours.}
However, translating structural side information into appropriate constraints for such algorithms requires further research. 
{\color{blue}It is worth mentioning that (Korhonen and Parviainen 2015) proposed a score-based method for learning bounded treewidth BNs with exponential complexity. We show in our work that such BN can be learned using constraint-based methods with polynomial complexity. }
For instance, the reviewer suggests an interesting idea for translating diamond-freeness into score-based algorithms. This translation and comparing their performances with our constraint-based method require further research and it is out of scope of this work.
\end{itemize}


\subsection*{Reviewer 3:}
\textbf{Summary:}
This paper discusses an approach for learning the structure of Bayesian networks using structural side information. In particular, the authors consider two types of structural information: (1) the network is diamond-free and (2) an upper bound on the clique number. To this end, the authors develop a new type of structure learning algorithm which they name "recursive structure learning", a constraint-based approach that recursively identifies separating sets in the graph. It is shown that this algorithm has a favourable computational complexity / running time compared to other structure learning methods. Furthermore, the algorithm performs well on a number of datasets in terms of predicting the correct edges.
\\
\\
\textbf{Main Review:}
The motivation for the types of structural information is not very strong in my opinion. There is a theoretical argument that such structural assumptions occur frequently in random Erdos-Renyi graphs, but in my experience, BNs in real life are often not diamond-free. There is also prior work on learning graphs with bounded treewidth, which is arguably more useful, because that determines the computational complexity of reasoning (which is ignored in this paper). I also think it is hard to imagine situations where one might want to learn the structure of a network, but where an upper bound on the clique number is known.

The experiments are interesting, in particular it is interesting to see that the approach also works quite well on the network with diamonds (Andes). Overall, the $RSL_D$ approach seems to work well, though sometimes MARVEL is better. I did not have some questions:

Somewhat of a weak point in the experiments are the selected networks: The bnlearn repository also has other networks of similar size. What was the criterion for selecting exactly these six networks? Did you test other networks as well?
I would think that in practice you would choose the upper bound on the clique number "large", at least sufficiently large to make sure that you do not underfit the structure. How would the approach compare to approaches in that case?
Overall, RSL seems a promising approach for fast structure learning. Given the questions about the practical usability of the method and weaknesses in the experimental methodology I cannot recommend acceptance at this point.
\\
\\
\textbf{Limitations And Societal Impact:}
There are no negative societal impacts to be expected. The paper does not discuss limitations beyond the assumptions the method uses.
\\
\\
\textbf{Ethical Concerns:}
No ethical issues.
\\
\\
\textbf{Needs Ethics Review:} No
\\
\\
\textbf{Time Spent Reviewing:} 2
\\
\\
\textbf{Rating:} 4: Ok but not good enough - rejection
\\
\\
\textbf{Confidence:} 3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.
\\
\\
\textbf{Code Of Conduct:} While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.


\subsection*{Detailed response to Reviewer 3 \& corresponding changes:}

Regarding the reviewer's concern about the motivation of our assumptions and also to address the first question:

\begin{itemize}
    \item 
As the reviewer mentioned, we have studied two structural side information: diamond-free and boundedness of the clique number. 
As we argue in Section 7 {\color{blue}(Section 6 in our NeurIPS21 submission)} about random graphs, sparse structures are diamond-free with high probability. 
Note that even $K_4$ ({\color{blue}complete graph with four vertices}) is a diamond-free graph, i.e., very dense graphs can also be diamond-free. Moreover, such structures appear frequently in many real-world applications. For instance, we observed this in the main database frequently used to study BNs (https://www.bnlearn.com/bnrepository/). We randomly selected 17 structures from this website for our experiments and observed that 15 were diamond-free. 
Even if the graph is not diamond-free, $RSL_D$ does not necessarily make a mistake. {\color{blue} We added section C in Appendix in which we explain this property in detail}. 
It is still highly likely that $RSL_D$ will choose the right node to remove and learn the structure with no errors (as witnessed by the example of Andes in our experiments). 
It is also worth mentioning that diamond-free graphs are a type of planar graphs that are well-studied in graph theory and possess interesting properties, e.g., while the coloring problem in general graphs is NP-hard, for diamond-free graphs is polynomial-time solvable. This work shows that the complexity of structure learning for such graphs is again polynomial in the number of variables.
 {\color{blue}
 We emphasized these facts in the AAAI-22 submission, Section 6.
 }


\item
We show that side information on the clique number of the graph reduces the learning complexity. It is important to emphasize that our proposed algorithm $RSL_\omega$ can verify the correctness of the bound on the clique number. Therefore, even if the clique number is not known, we can run $RSL_\omega$ with an initial guess about the clique number of the underlying BN. If the clique number of the output graph is less than the initial guess, the graph is learned correctly; otherwise, we need to increase our guess (Thus, as a side product, $RSL_\omega$ can identify the clique number of the underlying structure).
{\color{blue} We added Section 5 in our new submission in which we explain the verifiability of $RSL_\omega$ in Proposition 4 and develop Algorithm 5 that does not require any side information.}
 
 \item
 We appreciate the insightful comment about the relationship between our assumption on the clique number and the treewidth in (Elidan and Gould 2008, Korhonen and Parviainen 2015). In fact, we should emphasize that our work \textit{generalizes} the assumption on the treewidth. This is because, in general, the clique number is less than treewidth+1. Hence, having a bound on the treewidth of the underlying structure will lead to a bound on the clique number, and consequently (based on the result of Theorem 2), our algorithm will also have bounded complexity. On the other hand, a bound on the clique number does not translate to a bound in the correct direction for the treewidth. Therefore, the algorithm proposed in (Elidan and Gould 2008) cannot learn the graph with any guarantee. We also emphasize that the algorithm in (Elidan and Gould 2008, Korhonen and Parviainen 2015) requires knowledge of the treewidth, but as we mentioned above, $RSL_\omega$ can identify the structure without knowing the clique number but by progressively guessing and learning it.
{\color{blue} In our AAAI-22 submission, we rigorously explained the relationship between bounded treewidth assumption and our bounded clique number side information in the Introduction section and Related work. Moreover, we added more details on how our proposed $RL_\omega$ can learn bounded treewidth BNs and compared its complexity with the state-of-the-art exact and heuristic algorithms in Related work.
}
\end{itemize}

To address the second question raised by the reviewer:
\begin{itemize}
    \item 
We tested the algorithms on most of the graphs in the bnlearn repository, and the results were similar. We selected 5 of them due to the space restriction. Moreover, we chose these graphs to cover a wide range of variables (27, 70, 104, 223, 441), {\color{blue}see Table 4 in Appendix F}. To have a more comprehensive comparison, {\color{blue} we added Figure 3 in the main text and also Figure 6 in Appendix F, where we study the effect of sample size on learning performances of various algorithms for 4 different real world BNs.}\textcolor{red}{refer also to the figure with the effect of significance level}

\end{itemize}


\subsection*{Reviewer 4:}
\textbf{Summary:}
The paper describes a structural learning algorithm fro bayesian netwoks, in particular a constraint-based algorithm under the assumption that two different types of side information are vailable to the learner. Two specific types of side information are taken into account, namely the fact that the BN model is free from a specific structure named diamond and a secod type of side information represented by the knowledge of an upper bound for the number of cliques of the BN. The paper develops algorithms exploiting such particular type of side informations to efficiently learn the stricture of a BN from the available data. The paper desribes a set of numeicla experiments on both synthetic data, with specicic reference to a particular class of graphs and real world datasets which are typically used to compare structural learning algoritms.
\\
\\
\textbf{Main Review:}
Originality: The paper is somewhat original because it proposes new algorithms to learn the structure of bayesian networks from available data under teh paticular conition where side information is available.

Quality: The paper is of good quality, technical aspects are well managed and presented. However, I would have appreciated the paper to take into account also which is the impact of the available informatin on score based algoriths. Even if this is not a lack of the paper but comething that would have used to better quantify the quality of the developed algorithms. Technical details, lemmas and theorems are sound even if I personally did not check whether their proof is correct.

Clarity: The paper is clear, in other terms it is is clear the theoretical problem which is tackled and it is also very clear how the problem has been solved. However, I think that more time should be devoted to discuss limitations of the proposed approach. Also the description of the results of the performed numerical experiments is limited in my humble opinion. In parricular, I do not agree with the papers stating that accuracy of the proposed algorithms is superior in the case of the real worls datasets. Indeed, in 4 out of 6 I can not see any superiority, they behave like othe state of the art algorithms in terms ofF1. Additionally, I personally can not well understand what does it mean to compare algorithms which exploit side information to algorithms not exploiting such information, at least in terms of computational time. Itshould be clear that using additional and very strong assumptions in terms of side information the complexity of the developed algorithm will be better

Significance: I'm not convinced of the tru relevace of the proposed algorithms. Indeed, I can not quantify, extimate (my fault for sure, which is the potential exploitation of the developed algorithms, the diamond free and the knowledge of the upper bound of the number of cliques seem to be strong assumptions. SO I would appreciate very much whetehr the authors could help me to reduce my ignorance on the subject.
\\
\\
\textbf{Limitations And Societal Impact:}
Reading carefully more than three times the paper, I was not able to find any discussion about limitations and cirticism of the proposed algorithms. I also think that it could be interesting to evauate which could be the interplay between the two type of side effects.
\\
\\
\textbf{Ethical Concerns:}
NA
\\
\\
\textbf{Needs Ethics Review:} No
\\
\\
\textbf{Time Spent Reviewing:} 11
\\
\\
\textbf{Rating:} 4: Ok but not good enough - rejection
\\
\\
\textbf{Confidence:} 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
\\
\\
\textbf{Code Of Conduct:} While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.


\subsection*{Detailed response to Reviewer 4 \& corresponding changes:}
Clarification:

Based on the reviewer's summary, we believe there is a misunderstanding regarding our assumption for 
$RSL_\omega$ algorithm. Our assumption is that we have an upper bound for the clique number of the graph, not the number of cliques in the graphs.

Regarding the reviewer's comments on Significance:
\begin{itemize}
\item 
Our proposed algorithm 
$RSL_\omega$
 can verify the correctness of the bound on the clique number. Therefore, even if there is no information about the underlying clique number, we can run $RSL_\omega$ with an initial guess about the clique number of the underlying BN, and if the clique number of the output graph is less than the initial guess, then the graph is correct; otherwise, we need to increase our guess.
 {\color{blue} We added Section 5 in our new submission in which we explain the verifiability of $RSL_\omega$ in Proposition 4 and develop Algorithm 5 that does not require any side information.}


\item
Assuming an upper bound on the clique number of the underlying graph is less restrictive than other common assumptions in score-based methods such as an upper bound on the treewidth of the underlying graph (Elidan and Gould 2008, Korhonen and Parviainen 2015). This is because, in general, the clique number is less than treewidth+1. Hence, having a bound on the treewidth will lead to a bound on the clique number, and consequently (based on the result of Theorem 1), our algorithm will also have bounded complexity.
{\color{blue} In our AAAI-22 submission, we rigorously explained the relationship between bounded treewidth assumption and our bounded clique number side information in Section 1. Moreover, we added more details on how our proposed $RL_\omega$ can learn bounded treewidth BNs and compared its complexity with the state-of-the-art exact and heuristic algorithms in Related work.
}

\item 
As we argue in Section 7 {\color{blue}(Section 6 in our NeurIPS-21 submission)} about random graphs, sparse structures are diamond-free with high probability. 
Note that even $K_4$ ({\color{blue}complete graph with four vertices}) is a diamond-free graph, i.e., very dense graphs can also be diamond-free. Moreover, such structures appear frequently in many real-world applications. For instance, we observed this in the main database frequently used to study BNs (https://www.bnlearn.com/bnrepository/). We randomly selected 17 structures from this website for our experiments and observed that 15 were diamond-free. 
Even if the graph is not diamond-free, $RSL_D$ does not necessarily make a mistake. {\color{blue} We added section C in Appendix in which we explain this property in detail}. 
It is still highly likely that $RSL_D$ will choose the right node to remove and learn the structure with no errors (as witnessed by the example of Andes in our experiments). 
It is also worth mentioning that diamond-free graphs are a type of planar graphs that are well-studied in graph theory and possess interesting properties, e.g., while the coloring problem in general graphs is NP-hard, for diamond-free graphs is polynomial-time solvable. This work shows that the complexity of structure learning for such graphs is again polynomial in the number of variables.
 {\color{blue}
 We emphasized these facts in our AAAI-22 submission, Section 6.
 }
 
 \end{itemize}
 
 
Regarding the reviewer's comment about the limitations of the paper:
\begin{itemize}
    \item 
Thanks for the suggestion. \textcolor{blue}{We mentioned the restrictions of the algorithms more clearly, for instance, in the last paragraph of section 6, we discussed the limitations of $RSL_D$.} 
It is important to emphasize that our structural assumptions are our limitations. For example, we need the diamond-free assumption for the 
$RSL_D$ algorithm to be sound. 
%We also argue that this assumption is not verifiable (although we show that this assumption holds with high probability in sparse random graphs and many real-world structures. 
Moreover, we show that even if this assumption does not hold and the graph includes diamonds, there are only some rare cases when the algorithm makes mistakes, where such mistakes are only limited to some extra edges.
 {\color{blue} We added section C in Appendix in which we explain this property in detail and prove in Proposition 11 that $RSL_D$ has no false negative.}

\end{itemize}

Regarding the reviewer's comments about Clarity:


\begin{itemize}
    \item 
As depicted in Figure 2.a, 
$RSL_D$
 outperforms all the algorithms in terms of time complexity and accuracy. It seems that for graphs that are not very sparse, although the graph might contain diamonds, 
$RSL_D$
 outperforms the others. One justification for this robustness is that when the graph is not diamond-free, the event that 
$RSL_D$
 makes a mistake is quite rare. Moreover, in case of a mistake, 
$RSL_D$ outputs only a few extra edges in the graph. {\color{blue}To support our claim more rigorously, we added section C in Appendix in which we explain this property in detail and prove in Proposition 11 that $RSL_D$ has no false negative.}

\item
As mentioned by the reviewer, we compared our algorithms that use two types of structural assumptions (although 
$RSL_\omega$
 can still work without any assumption) with other algorithms that do not use this information. This is the primary purpose of this paper. Learning the structure of BNs, in general, is NP-hard and requires an exponential number of CI tests in the worst-case. This paper shows that the structure learning problem with extra structural assumptions can be solved in polynomial time. Our experiments presented in Section 8 {\color{blue} (Section 7 of our NeurIPS-21 submission)} also advocate that our algorithms can efficiently incorporate such structural assumptions.

\end{itemize}

{\color{blue}
\subsection*{NeurIPS-21 reviews quality:}
 We believe that the review quality of Reviewer 4 is not satisfactory, and he/she does not provide a meaningful assessment of our work. 
 Moreover, Reviewer 3 and 4 did not respond to our author responses. 

To back up our claim, we point you to the reviewer's comments that contain many grammatical errors and typos. This makes them hard to understand and sometimes meaningless, e.g.,

\textit{``... could be interesting to evauate which could be the interplay between the two type of side effects.''}
or

 \textit{``I'm not convinced of the tru relevace of the proposed algorithms. Indeed, I can not quantify, extimate (my fault for sure, which is the potential exploitation of the developed algorithms, the diamond free and the knowledge of the upper bound of the number of cliques seem to be strong assumptions. SO I would appreciate very much whetehr the authors could help me to reduce my ignorance on the subject.''}
Also, based on the reviewer's summary, the reviewer did not understand our main assumption that is an upper bound on the clique number, not on the number of cliques.

Another point is that the whole idea of our paper is to show that side information can reduce the complexity of structure learning. Hence, we compared our proposed algorithms with the state-of-the-art algorithms that ignore such information. However, the reviewer sees this comparison as a negative point of our work:

\textit{``I personally can not well understand what does it mean to compare algorithms which exploit side information to algorithms not exploiting such information, at least in terms of computational time. It should be clear that using additional and very strong assumptions in terms of side information the complexity of the developed algorithm will be better''}


}



==> coverletter_final.tex <==
\clearpage

\section*{Cover Letter}

We first address a main concern which was common among the reviewers regarding the motivations for our structural assumptions, as we did not discuss certain important motivations for these assumptions in our NeurIPS submission.
For instance, the exact connection between our assumption to the problem of learning BNs with bounded treewidth, which recently has gained a lot of attention in the literature, was not discussed in detail. 
Below, we discuss our main motivations and how we edited the paper accordingly. 

\paragraph{Assuming an upper bound on the clique number:}
\begin{itemize}
    \item \textbf{Treewidth + 1 $\leq \omega$ }: 
        In our AAAI-22 submission, we rigorously explained the relationship between bounded treewidth assumption and our bounded clique number side information in the Introduction section and Related work. Moreover, we added more details on how our proposed $RSL_\omega$ can learn bounded treewidth BNs and compared its complexity with the state-of-the-art exact and heuristic algorithms in Related work.
        We emphasize that our work \textit{generalizes} the assumption on the treewidth. This is because, in general, the clique number is less than treewidth+1. Hence, having a bound on the treewidth of the underlying structure will lead to a bound on the clique number, and consequently (based on the result of Theorem 1), our algorithm will also have bounded complexity. On the other hand, a bound on the clique number does not translate to a bound in the correct direction for the treewidth. Therefore, the algorithm proposed in (Elidan and Gould 2008) cannot learn the graph with any guarantee. We also emphasize that the algorithm in (Elidan and Gould 2008, Korhonen and Parviainen 2015) requires knowledge of the treewidth, but $RSL_\omega$ can identify the structure without knowing the clique number but by progressively guessing and learning it.
    \item \textbf{RSL$_\omega$ is verifiable (Section \ref{sec: without side information})}:
        We have added a new section to the AAAI submission to discuss that our proposed algorithm $RSL_\omega$ can verify the correctness of the bound on the clique number (Proposition 4) and therefore, it can be used to learn a BN without any side information (Algorithm \ref{alg: without side information}). Because, even if the clique number is not known, we can run $RSL_\omega$ with an initial guess about the clique number of the underlying BN. If the clique number of the output graph is less than the initial guess, the graph is learned correctly; otherwise, we need to increase our guess.
\end{itemize}

\paragraph{Diamond-free assumption:}
\begin{itemize}
    \item \textbf{No false negative (Appendix C):}
        Although we proved the correctness of $RSL_D$ under the assumption that the true BN is diamond-free, $RSL_D$ does not necessarily make a mistake if the graph contains diamonds.
        Even in the case of a BN with diamonds, it is still highly probable that $RSL_D$ will choose the right node to remove and learn the structure with no errors (see the example in Appendix C for further discussion.)
        This was also witnessed in practice in the example of Andes structure in our experiments (see Figure \ref{fig: Andes} and Table \ref{table: real-world}), which contains diamonds and yet, $RSL_D$ demonstrates the best accuracy among the cohort.
        Moreover, in case of a mistake, 
        $RSL_D$ outputs only a few extra edges in the graph. To support our claim more rigorously, we added section C in Appendix, in which we explain this property in detail and prove in \textbf{Proposition 11} that $RSL_D$ has no false negative.
    \item \textbf{Random graphs:}
        As we argue in Section 7 (Section 6 in the NeurIPS-21 submission) about random Erdos-Renyi graphs, sparse structures are diamond-free with high probability. 
        Note that even $K_4$ (complete graph with four vertices) is a diamond-free graph, i.e., very dense graphs can also be diamond-free.
        
    \item\textbf{Experimental results (Section 8, Appendix F)}
        For the AAAI submission, we added discussions in Section 8 and Appendix F about the performance of RSL$_D$. 
        There, we showed that RSL$_D$ outperforms various algorithms in terms of both time complexity and accuracy in most of the cases, which supports its practical usability.
    \item \textbf{Real-world structures are often diamond-free (Appendix F):}
        Diamond-free structures frequently appear in many real-world applications. For instance, we observed this in the main database frequently used to study BNs (https://www.bnlearn.com/bnrepository/. We randomly selected 17 structures from this website for our experiments and observed that 15 out of these 17 structures were diamond-free. 
        This is to support that although the diamond-freeness might seem a strong assumption, it is applicable in many real-world applications with no concern.
        \item
        It is also worth mentioning that diamond-free graphs are a type of planar graphs that are well-studied in graph theory and possess interesting properties, e.g., while various problems such as the coloring problem, maximum weight stable set, maximum weight clique, and domination in general graphs are NP-hard, for diamond-free graphs are polynomial-time solvable. This work shows that the complexity of structure learning for such graphs is again polynomial in the number of variables.
        We emphasized these facts in our AAAI-22 submission, \emph{Section 6}.
\end{itemize}


% As depicted in Figure 2.a, 
% $RSL_D$
%  outperforms all the algorithms in terms of time complexity and accuracy. It seems that for graphs that are not very sparse, although the graph might contain diamonds, 
% $RSL_D$
%  outperforms the others. One justification for this robustness is that when the graph is not diamond-free, the event that 
% $RSL_D$
%  makes a mistake is quite rare. Moreover, 

Next, we address other concerns raised specifically by each reviewer.
\subsection*{Reviewer 1 (T1fT)}
Experiments:
\begin{itemize}
    \item Large dataset size (50n): We added new experiments to illustrate the effect of sample size. For instance, we added Figure 3 in the main text and Figure 5 in Appendix F where the horizontal axis is the number of samples. Also, we added Figure 2e where the sample size is $20n$, unlike figure 2d where the sample size is $50n$.
    
    \item
    Confidence intervals: As mentioned in Section 8, "Each point is reported as the average of 100 runs, and the shaded areas indicate the 80\% confidence intervals." 
% Performance of various methods: As depicted in Figure 2.a, 
% $RSL_D$ outperforms all the algorithms in terms of time complexity and accuracy. 
% It seems that for graphs that are not very sparse, although the graph might contain diamonds, 
% $RSL_D$ outperforms the others. One justification for this robustness is that when the graph is not diamond-free, the event that 
% $RSL_D$ makes a mistake is quite rare. Moreover, in case of a mistake, 
% $RSL_D$ outputs only a few extra edges (It does not miss any edges) in the graph. {\color{blue}To support our claim more rigorously, we added Proposition 11 in the Appendix C that shows even if the underlying BN contains diamonds, the output of $RSL_D$ does not miss any edges i.e.,  $RSL_D$ has recall one.}
\end{itemize}

Regarding Clarity:
\begin{itemize}
    \item Last paragraph of Section 6 (Section 4 of our NeurIPS21 submission): We proved the correctness of Algorithm 4 under the assumption that the underlying structure is diamond-free in Theorem 2 (Theorem 1 in our NeurIPS21 submission). 
    However, when the assumption is not valid, the output of Algorithm $RSL_D$ is not necessarily incorrect. More precisely, RSL makes a mistake when either Algorithm 3 incorrectly reports a node as removable or Algorithm 4 identifies the wrong neighbors. For example, Algorithm 3 selects a wrong removable in the left graph in Figure 1 (this graph violates the diamond-free assumption) only when A is selected in the first iteration. Note that this happens with a probability 0.25 since all the variables have the same Markov boundary size. Another example is the right graph in Figure 1, in which Algorithm 3 works without error (all the variables are truly removable) but Algorithm 4 incorrectly identifies the neighbors only when nodes B or C are selected by Algorithm 3 in the first iteration. This occurs with a probability 0.5. 
    In the last paragraph of Section 6 of our AAAI-22 submission, we briefly explained the aforementioned notes to avoid any ambiguity. 
    Further, we added more details in Section C of Appendix, including Proposition 11, which proves that $RSL_D$ has no false negative. 

\end{itemize}


\subsection*{Reviewer 2 (CUxT)}
The text in grey is quoted from the reviewer.
\begin{itemize}
    \item 
{\color{gray}\textit{The various algorithms are presented with an unstated assumption that we are doing oracle-based learning. For example, as noted in the "Problem description" section we do not learn from $P_V$
, but from a finite sample drawn from $P_V$
. So it is a ... I think some small alteration to the presentation could fix this.}}

As the reviewer correctly mentioned, structural learning is from data, not the probability distribution in practice. However, in the theoretical part, we present our algorithms and results under the assumption that we have access to an infinite number of sample points or the true joint distribution equivalently. 
We emphasized this in \textbf{Section \ref{sec: RSL} (footnote 6)} that in practice, the finite sample data at hand is used instead of $P_{\OV}$.


\item 
{\color{gray}\textit{There is no empirical comparison of the effect of different significance levels: they always use 0.01 (and $2/n^2$ for Markov blanket "discovery" - actually estimation).}}

We ran the algorithms for a wide range of significance levels, and the numbers around 0.01-0.05 work best for almost all the Algorithms. 
We have included the \textbf{Figure 7 in Appendix F} to support the fact that the choice of significance level does not alter the experimental results significantly.
We also note that this choice of the significance level is common in constraint-based methods. Also, as discussed in reference (Pellet and Elis- seeff 2008) of the paper, $2/n^2$ is a good choice for Markov boundary discovery.

\item 
{\color{gray}\textit{``Runtime and the number of CI tests are reported after Markov boundary discovery''. It would be good to know how long Markov boundary estimation takes.}}


Since all the methods require Markov boundary, and we used a similar method for all of them, the runtime is the same. However, In the method that we used in our experiments, the number of CI tests is always $\binom{n}{2}$, and as suggested by the reviewer, we reported the runtime for computing Markov boundaries for one of our experiments in \textbf{Figure 6 in Appendix F}.

\item
{\color{gray}\textit{In any score-based approach which had binary variables for both parent sets and adjacencies in the DAG, one would rule out diamonds with simple linear constraints as follows: I(D<-{A,B,C}) + I(A-B) + I(A-C) <= 2 + I(B-C) If cliques of size 4 (and above) were not allowed, ... it would be interesting to see.}}


We appreciate the insightful comment of the reviewer. Certain score-based algorithms are capable of incorporating structural side information.
We have reviewed a few such score-based methods that are related to our work in our AAAI-22 submission and compared their assumptions and complexity with ours.
However, translating structural side information into appropriate constraints for such algorithms requires further research. 
It is worth mentioning that (Korhonen and Parviainen 2015) proposed a score-based method for learning bounded treewidth BNs with exponential complexity. We show in our work that such BN can be learned using constraint-based methods with polynomial complexity. 
For instance, the reviewer suggests an interesting idea for translating diamond-freeness into score-based algorithms. This translation and comparing their performances with our constraint-based method require further research and it is out of the scope of this work.
\end{itemize}

\subsection*{Reviewer 3 (NGjF)}

To address the second question raised by the reviewer:
\begin{itemize}
    \item 
    We tested the algorithms on most of the graphs in the bnlearn repository, and the results were similar. We selected 5 of them due to the space restriction. Moreover, we chose these graphs to cover a wide range of variables (27, 70, 104, 223, 441), see Table 4 in Appendix F. To have a more comprehensive comparison, we added Figure 3 in the main text and also Figures 6 and 7 in Appendix F.
    In these figures we study the effect to sample size and significance level of the performed CI tests for 5 different real-world BNs.
\end{itemize}

\subsection*{Reviewer 4 (yAbM)}

Based on the reviewer's summary, we believe there is a misunderstanding regarding our assumption for 
$RSL_\omega$ algorithm. Our assumption is that we have an upper bound for the clique number of the graph, not the number of cliques in the graphs.

 
 
Regarding the reviewer's comment about the limitations of the paper:
\begin{itemize}
    \item 
    We mentioned the restrictions of the algorithms more clearly; for instance, in the last paragraph of section 6, we discussed the limitations of $RSL_D$.
    It is important to emphasize that our structural assumptions are our limitations. For example, we need the diamond-free assumption for the $RSL_D$ algorithm to be sound. 
    Moreover, we show that even if this assumption does not hold and the graph includes diamonds, there are only rare cases when the algorithm makes mistakes, where such mistakes are only limited to a few extra edges.
    We added Appendix C, in which we explain this property in detail and prove in Proposition 11 that $RSL_D$ has no false negative.
\end{itemize}

Regarding the reviewer's comments about Clarity:


\begin{itemize}
%     \item 
% As depicted in Figure 2.a, 
% $RSL_D$
%  outperforms all the algorithms in terms of time complexity and accuracy. It seems that for graphs that are not very sparse, although the graph might contain diamonds, 
% $RSL_D$
%  outperforms the others. One justification for this robustness is that when the graph is not diamond-free, the event that 
% $RSL_D$
%  makes a mistake is quite rare. Moreover, in case of a mistake, 
% $RSL_D$ outputs only a few extra edges in the graph. {\color{red}To support our claim more rigorously, we added section C in Appendix in which we explain this property in detail and prove in Proposition 11 that $RSL_D$ has no false negative.}

\item
As mentioned by the reviewer, we compared our algorithms that use two types of structural assumptions (although 
$RSL_\omega$
 can still work without any assumption) with other algorithms that do not use this information. This is the primary purpose of this paper. Learning the structure of BNs, in general, is NP-hard and requires an exponential number of CI tests in the worst-case. This paper shows that the structure learning problem with extra structural assumptions can be solved in polynomial time. Our experiments presented in Section 8 (Section 7 of our NeurIPS-21 submission) also advocate that our algorithms can efficiently incorporate such structural assumptions.

\end{itemize}


\subsection*{On the review of reviewer 4 (yAbM):}
We believe that the review quality of Reviewer 4 is not satisfactory, and he/she does not provide a meaningful assessment of our work.
% Moreover, Reviewers 3 and 4 did not respond to our author responses. 
To back up our claim, we point you to the reviewer's comments that contain many grammatical errors and typos. This makes them hard to understand and sometimes meaningless, e.g.,

{\color{gray}\textit{``... could be interesting to evauate which could be the interplay between the two type of side effects.''}}

or

{\color{gray}\textit{``I'm not convinced of the tru relevace of the proposed algorithms. Indeed, I can not quantify, extimate (my fault for sure, which is the potential exploitation of the developed algorithms, the diamond free and the knowledge of the upper bound of the number of cliques seem to be strong assumptions. SO I would appreciate very much whetehr the authors could help me to reduce my ignorance on the subject.''}}

Also, based on the reviewer's summary, the reviewer did not understand our main assumption that is an upper bound on the clique number, not on the number of cliques.

Another point is that the whole idea of our paper is to show that side information can reduce the complexity of structure learning. Hence, we compared our proposed algorithms with the state-of-the-art algorithms that ignore such information. However, the reviewer sees this comparison as a negative point of our work:

{\color{gray}\textit{``I personally can not well understand what does it mean to compare algorithms which exploit side information to algorithms not exploiting such information, at least in terms of computational time. It should be clear that using additional and very strong assumptions in terms of side information the complexity of the developed algorithm will be better''}}.

